A Snapshot Survey of Nearby Supernovae with the Hubble Space Telescope

Over recent decades, robotic (or highly automated) searches for supernovae (SNe) have discovered several thousand events, many of them in quite nearby galaxies (distances < 30 Mpc). Most of these SNe, including some of the best-studied events to date, were found before maximum brightness and have associated with them extensive follow-up photometry and spectroscopy. Some of these discoveries are so-called SN impostors, thought to be superoutbursts of luminous blue variable stars, although possibly a new, weak class of massive-star explosions. We conducted a Snapshot program with the Hubble Space Telescope(HST) and obtained images of the sites of 31 SNe and four impostors, to acquire late-time photometry through two filters. The primary aim of this project was to reveal the origin of any lingering energy for each event, whether it is the result of radioactive decay or, in some cases, ongoing late-time interaction of the SN shock with pre-existing circumstellar matter, or the presence of a light echo. Alternatively, lingering faint light at the SN position may arise from an underlying stellar population (e.g., a host star cluster, companion star, or a chance alignment). The results from this study complement and extend those from Snapshot programs by various investigators in previous HST cycles.

==> Figure_set.tex <==
\figsetstart
\figsetnum{1}
\figsettitle{SN lightcurve/finder charts combined}
\figsetgrpstart
\figsetgrpnum{figurenumber.1}
\figsetgrptitle{SN 2010jl}
\figsetplot{SN_2010jl_combined}
\figsetgrpnote{Finder chart and lightcurve for SN 2010jl. "Other" data shown are from \citet{Ofek2014} and \citet{Jencson2016}. Other HST F336W and F814W datapoints are from \citet{Fox2017} and data from G0-15166.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.2}
\figsetgrptitle{SN 2010mc}
\figsetplot{SN_2010mc_combined}
\figsetgrpnote{Finder chart and lightcurve for SN 2010mc. "Other" data shown are from \citet{Ofek2013} and \citet{Smith2014}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.3}
\figsetgrptitle{SN 2011dh}
\figsetplot{SN_2011dh_combined}
\figsetgrpnote{Finder chart and lightcurve for SN 2011dh.Lick data shown are from \citet{Zheng2022}, and other data are from \citet{Arcavi2011}, \citet{Tsvetkov2012},\citet{Sahu2013},\citet{Marion2014} and \citet{Ergon2015}. HST data are from \citet{Maund2015} and \citet{Maund2019} as well as programs G)-15645 and GO-16024.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.4}
\figsetgrptitle{SN 2012A}
\figsetplot{SN_2012A_combined}
\figsetgrpnote{Finder chart and lightcurve for SN 2012A. Given the non-detection, the location is denoted by a dashed circle. Lick data shown are from \citet{deJaeger2019}, and other data are from \citet{Tomasella2013}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.5}
\figsetgrptitle{SN 2012aw}
\figsetplot{SN_2012aw_combined}
\figsetgrpnote{Finder chart and lightcurve for SN 2012aw.Lick data shown are from \citet{deJaeger2019}, and other data are from \citet{Spogli2020}.\citet{Bose2013} and \citet{Dall'Ora2014}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.6}
\figsetgrptitle{SN 2013df}
\figsetplot{SN_2013df_combined}
\figsetgrpnote{Finder chart and lightcurve for SN 2013df.Lick data shown are from \citet{VanDyk2014}, and other data are from \citet{Morales2014} and \citet{Szalai2016}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.7}
\figsetgrptitle{SN 2013ej}
\figsetplot{SN_2013ej_combined}
\figsetgrpnote{Finder chart and lightcurve for SN 2013ej.Lick data shown are from \citet{deJaeger2019}, and other data are from \citet{Richmond2014},\citet{Bose2015}, \citet{Huang2015},\citet{Dhungana2016},\citet{Yuan2016} and \citet{Mauerhan2017}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.8}
\figsetgrptitle{SN 2014C}
\figsetplot{SN_2014C_combined}
\figsetgrpnote{Finder chart and lightcurve for SN 2014C.Lick data shown are from \citet{Zheng2022}, and our HST data is augmented by GO-14668 and GO-15166 as well as data from \citet{Sun2020}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.9}
\figsetgrptitle{SN 2015cp}
\figsetplot{SN_2015cp_combined}
\figsetgrpnote{Finder chart and lightcurve for SN 2015cp. Given the non-detection, the location is denoted by a dashed circle. The other optical data shown is the iPTF R lightcurve as well as one rereduced HST F275W points from \citet{Graham2019}}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.10}
\figsetgrptitle{SN 2016G}
\figsetplot{SN_2016G}
\figsetgrpnote{Finder chart and lightcurve for SN 2016G.Given the non-detection, the location is denoted by a dashed circle. The lick data is from \citet{Zheng2022}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.11}
\figsetgrptitle{SN 2016adj}
\figsetplot{SN_2016adj}
\figsetgrpnote{Finder chart and lightcurve for SN 2016G.Given the non-detection, the location is denoted by a dashed circle. Also shown are \citet{Stritzinger2022} and \citet{Stritzinger2023} data which analyzed the readily apparent light echo.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.12}
\figsetgrptitle{SN 2016bkv}
\figsetplot{SN_2016bkv}
\figsetgrpnote{Finder chart and lightcurve for SN 2016bkv. The Lick data is previously unpublished, and other data comes from \citet{Nakaoka2018} and \citet{Hosseinzadeh2018}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.13}
\figsetgrptitle{AT 2016blu}
\figsetplot{AT_2016blu}
\figsetgrpnote{Finder chart and lightcurve for SN impostor AT 2016blu. The Lick data shown was used in \citet{Aghakhanloo2022b}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.14}
\figsetgrptitle{SN 2016coi}
\figsetplot{SN_2016coi}
\figsetgrpnote{Finder chart and lightcurve for SN 2016coi.Given the non-detection, the location is denoted by a dashed circle. The Lick data shown are from  \citet{Zheng2022}. "Other" data are from \citet{Kumar2018},\citet{Terreran2019},\citet{Prentice2018} and \citet{Tsvetkov2020}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.15}
\figsetgrptitle{SN 2016coj}
\figsetplot{SN_2016coj}
\figsetgrpnote{Finder chart and lightcurve for SN 2016coj.Given the non-detection, the location is denoted by a dashed circle. The Lick data shown are from  \citet{Stahl2019}. "Other" data are from \citet{Richmond2017}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.16}
\figsetgrptitle{SN 2016gkg}
\figsetplot{SN_2016gkg}
\figsetgrpnote{Finder chart and lightcurve for SN 2016gkg.Given the F438W non-detection, the location is denoted by a dashed circle in one of the finder frames. The Lick data shown are from  \citet{Bersten2018} and \citet{Zheng2022}. "Other" data are from \citet{Tartaglia2017b}, with other HST data from \citet{Kilpatrick2022}}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.17}
\figsetgrptitle{SN 2016jbu}
\figsetplot{SN_2016jbu}
\figsetgrpnote{Finder chart and lightcurve for SN impostor AT 2016jbu.  "Other" data are from \citet{Kilpatrick2018b},\citet{Brennan2022a} with HST data combined with our data from \citet{Brennan2022b} and \citet{Brennan2022c}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.18}
\figsetgrptitle{SN 2016jbu}
\figsetplot{SN_2016jbu}
\figsetgrpnote{Finder chart and lightcurve for SN 2017cfd. Given the non-detection, the location is denoted by a dashed circle. Lick data are from \citet{Stahl2019}, and  "Other" data are from \citet{Han2020}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.19}
\figsetgrptitle{SN 2017eaw}
\figsetplot{SN_2016eaw}
\figsetgrpnote{Finder chart and lightcurve for SN 2017eaw.  Lick data are from \citet{VanDyk2019}, and  "Other" data are from \citet{Tsvetkov2020},\citet{Szalai2019b} and \citet{Buta2019}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.20}
\figsetgrptitle{SN 2017gax}
\figsetplot{SN_2017gax}
\figsetgrpnote{Finder chart and lightcurve for SN 2017gax.  Given the non-detection, the location is denoted by a dashed circle.  There is no photometry for this SN. }
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.21}
\figsetgrptitle{SN 2017gkk}
\figsetplot{SN_2017gkk}
\figsetgrpnote{Finder chart and lightcurve for SN 2017gkk.  The lightcurve contains unpublished Lick data, along with "other" data taken by \citet{Balanutsa2017}, \citet{Itagaki2017} and \citet{Vinko2017}. }
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.22}
\figsetgrptitle{SN 2017ixv}
\figsetplot{SN_2017ixv}
\figsetgrpnote{Finder chart and lightcurve for SN 2017ixv.  Given the non-detection, the location is denoted by a dashed circle.  There is no photometry for this SN. }
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.23}
\figsetgrptitle{SN 2018gj}
\figsetplot{SN_2018gj}
\figsetgrpnote{Finder chart and lightcurve for SN 2018gj. The lightcurve contains unpublished Lick data, along with "other" data taken by \citet{Teja2023} as well as our snapshots.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.24}
\figsetgrptitle{SN 2018zd}
\figsetplot{SN_2018zd}
\figsetgrpnote{Finder chart and lightcurve for SN 2018zd. Given the non-detection, the location is denoted by a dashed circle.  The lightcurve contains "other" data from \citet{Zhang2020}, \citet{Hiramatsu2021} and \citet{Callis2021} with HST data from \citet{Hiramatsu2021}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.25}
\figsetgrptitle{SN 2018aoq}
\figsetplot{SN_2018aoq}
\figsetgrpnote{Finder chart and lightcurve for SN 2018aoq. Given the non-detection, the location is denoted by a dashed circle.  The lightcurve contains previously unpublished Lick data ,as well as other data from\citet{ONeill2019} and \citet{Tsvetkov2019}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.26}
\figsetgrptitle{SN 2018cow}
\figsetplot{SN_2018cow}
\figsetgrpnote{Finder chart and lightcurve for SN 2018cow. The lightcurve contains Lick data from \citet{Zheng2022} ,as well as other data from\citet{Perley2019}, \citet{Margutti2019}, \citet{Xiang2021} and \citet{Tsvetkov2022}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.27}
\figsetgrptitle{SN 2018ivc}
\figsetplot{SN_2018ivc}
\figsetgrpnote{Finder chart and lightcurve for SN 2018ivc. The lightcurve contains unpublished Lick data,as well as other data from\citet{Bostroem2020} which includes data from HST program GO-15151.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.28}
\figsetgrptitle{SN 2019ehk}
\figsetplot{SN_2019ehk}
\figsetgrpnote{Finder chart and lightcurve for SN 2019ehk. Given the non-detection, the location is denoted by a dashed circle. The lightcurve contains unpublished Lick data,as well as other data from \citet{Nakaoka2021} and \citet{JacobsonGalan2021}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.29}
\figsetgrptitle{AR 2019krl}
\figsetplot{AT_2019krl}
\figsetgrpnote{Finder chart and lightcurve for SN impostor AT 2019krl. The lightcurve contains other data from \citet{Andrews2021}.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.30}
\figsetgrptitle{SN 2020dpw}
\figsetplot{SN 2020dpw}
\figsetgrpnote{Finder chart for SN impostor SN 2020dpw. There is no lightcurve data}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.30}
\figsetgrptitle{SN 2020hvp}
\figsetplot{SN 2020hvp}
\figsetgrpnote{Finder chart and lightcurve for SN impostor SN 2020hvp. The Lick data is previously unpublished.]}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.30}
\figsetgrptitle{SN 2020jfo}
\figsetplot{SN 2020jfo}
\figsetgrpnote{Finder chart and lightcurve for SN impostor SN 2020jfo The Lick data is from \citet{Ailawadhi2022}, and other data is from \citet{Sollerman2021} and \citet{Teja2022}.}
\figsetgrpend
\figsetend
\figsetstart
\figsetnum{2}
\figsettitle{Appendix Finder charts}
\figsetgrpstart
\figsetgrpnum{figurenumber.1}
\figsetgrptitle{SN 1999el+Sn 1999gi}
\figsetplot{99el_99gi_combined}
\figsetgrpnote{Finder charts for serendipitously caught SN's 1999el and 1999gi. As these SN were not detected, we note their location with dashed circles.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.2}
\figsetgrptitle{SN 2000E+2006X}
\figsetplot{00E_06X_combined}
\figsetgrpnote{Finder charts for serendipitously caught SN's 2000E and 2006X. Non-detections noted with a dashed circle.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.3}
\figsetgrptitle{SN 2006ov+2012bv}
\figsetplot{06ov_12bv_combined}
\figsetgrpnote{Finder charts for serendipitously caught SN's 2006ov and 2012bv. Non-detections noted with a dashed circle.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.4}
\figsetgrptitle{SN 2013ff+PSNJ09}
\figsetplot{13ff_PSNJO9}
\figsetgrpnote{Finder charts for serendipitously caught SN's 2013ff and PSN J09132750+7627410. Non-detections noted with a dashed circle.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.5}
\figsetgrptitle{SN 2015G+SN 2020oi}
\figsetplot{15G_20oi}
\figsetgrpnote{Finder charts for serendipitously caught SN's 2015G and 2020oi. Non-detections noted with a dashed circle.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.6}
\figsetgrptitle{SN 2021J+SN 2021sjt}
\figsetplot{21J_21sjt}
\figsetgrpnote{Finder charts for serendipitously caught SN's 2021J and 2021sjt. Non-detections noted with a dashed circle.}
\figsetgrpend
\figsetgrpstart
\figsetgrpnum{figurenumber.7}
\figsetgrptitle{SN 2022aau}
\figsetplot{22aau}
\figsetgrpnote{Finder charts for serendipitously caught SN 2022aau. Non-detections noted with a dashed circle.}
\figsetgrpend
\figsetend
